InstructEval: Systematic Evaluation of Instruction Selection Methods

In-context learning (ICL) performs tasks by prompting a large language model (LLM) using an instruction and a small set of annotated examples called demonstrations. Recent work has shown that precise details of the inputs used in the ICL prompt significantly impact performance, which has incentivized instruction selection algorithms. The effect of instruction-choice however is severely underexplored, with existing analyses restricted to shallow subsets of models and tasks, limiting the generalizability of their insights. We develop InstructEval, an ICL evaluation suite to conduct a thorough assessment of these techniques. The suite includes 13 open-sourced LLMs of varying scales from four model families, and covers nine tasks across three categories. Using the suite, we evaluate the relative performance of seven popular instruction selection methods over five metrics relevant to ICL. Our experiments reveal that using curated manually-written instructions or simple instructions without any task-specific descriptions often elicits superior ICL performance overall than that of automatic instruction-induction methods, pointing to a lack of generalizability among the latter. We release our evaluation suite for benchmarking instruction selection approaches and enabling more generalizable methods in this space.

==> figures/prompt_example_tikz.tex <==
\begin{tikzpicture}[
  node distance = 0.2cm and 0.2cm,
  single node/.style = {rectangle, fill=#1, fill opacity=0.5, text opacity=1, align=left, font=\fontfamily{FiraSans-LF}\selectfont\footnotesize, text width=0.40\textwidth, inner xsep=3mm, inner ysep=3mm, rounded corners=1mm},
]

\node[single node=lightyellow] (instruction) 
{\normalFont{Is this review positive or negative?}};

\node[single node=lightblue, below=of instruction] (example1)
{\normalFont{Review:} \ultraLight{Whoever wrote the screenplay for this movie obviously never consulted…} \\ \normalFont{Sentiment:} \ultraLight{Negative}};

\node[single node=lightblue, below=of example1] (example2)
{\normalFont{Review:} \ultraLight{The story centers around Barry McKenzie who must go to England…} \\ \normalFont{Sentiment:} \ultraLight{Positive}};

\node[single node=lightblue, below=of example2] (example3)
{\normalFont{Review:} \ultraLight{This film is just plain horrible. John Ritter doing pratt falls, 75\% of the actors…} \\ \normalFont{Sentiment:} \ultraLight{Negative}};


\node[single node=lightpink, below=of example3] (test) 
{\normalFont{Review:} \ultraLight{BLACK WATER has to be one of the best Australian movies I've seen in many…} \\ \normalFont{Sentiment:} };

\draw [black, line width=0.5pt, rounded corners=1mm] ([shift={(-2mm,-2mm)}]current bounding box.south west) rectangle ([shift={(2mm,2mm)}]current bounding box.north east);

\end{tikzpicture}

==> tables/all_results.tex <==
\onecolumn
\tiny
\tablefirsthead{%
\hline
dataset & model & method & Zero-shot accuracy & Few-shot accuracy & Perturbation accuracy & Selectional STD & Permutational STD \\
\hline}
\tablehead{%
\multicolumn{8}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline
dataset & model & method & Zero-shot accuracy & Few-shot accuracy & Perturbation accuracy & Selectional STD & Permutational STD \\
\hline}
\tabletail{%
\hline \multicolumn{8}{|r|}{{Continued on next page}} \\ \hline}
\tablelasttail{\hline}
\tablecaption{Results for all tasks, models, instruction selection/induction methods, and metrics}
\label{table:all_results}
\begin{supertabular}{lllrrrrr}
AG News & bloom1b1 & APE &            0.316 &           0.298 &          0.264 &        0.067 &    0.058 \\
              &        & Ad hoc &            0.592 &           0.537 &          0.463 &        0.145 &    0.111 \\
              &        & Generic Instruction &            0.636 &           0.609 &          0.543 &        0.140 &    0.121 \\
              &        & Low Perplexity &            0.656 &           0.472 &          0.400 &        0.135 &    0.112 \\
              &        & PromptSource &            0.600 &           0.490 &          0.425 &        0.136 &    0.118 \\
              &        & Null Instruction &            0.520 &           0.520 &          0.447 &        0.133 &    0.132 \\
              &        & RLPrompt &            0.672 &           0.554 &          0.480 &        0.140 &    0.137 \\
              & bloom1b7 & APE &            0.352 &           0.415 &          0.413 &        0.062 &    0.058 \\
              &        & Ad hoc &            0.492 &           0.610 &          0.549 &        0.084 &    0.088 \\
              &        & Generic Instruction &            0.564 &           0.631 &          0.552 &        0.092 &    0.087 \\
              &        & Low Perplexity &            0.456 &           0.542 &          0.493 &        0.105 &    0.089 \\
              &        & PromptSource &            0.612 &           0.585 &          0.530 &        0.084 &    0.091 \\
              &        & Null Instruction &            0.680 &           0.661 &          0.580 &        0.081 &    0.089 \\
              &        & RLPrompt &            0.636 &           0.649 &          0.567 &        0.086 &    0.092 \\
              & bloom3b & APE &            0.444 &           0.651 &          0.633 &        0.109 &    0.086 \\
              &        & Ad hoc &            0.600 &           0.791 &          0.756 &        0.033 &    0.039 \\
              &        & Generic Instruction &            0.628 &           0.803 &          0.763 &        0.035 &    0.031 \\
              &        & Low Perplexity &            0.444 &           0.783 &          0.735 &        0.049 &    0.051 \\
              &        & PromptSource &            0.616 &           0.793 &          0.750 &        0.041 &    0.040 \\
              &        & Null Instruction &            0.440 &           0.803 &          0.775 &        0.031 &    0.032 \\
              &        & RLPrompt &            0.692 &           0.801 &          0.763 &        0.030 &    0.033 \\
              & bloom7b1 & APE &            0.416 &           0.663 &          0.617 &        0.071 &    0.052 \\
              &        & Ad hoc &            0.560 &           0.785 &          0.740 &        0.039 &    0.045 \\
              &        & Generic Instruction &            0.780 &           0.795 &          0.753 &        0.037 &    0.040 \\
              &        & Low Perplexity &            0.620 &           0.767 &          0.713 &        0.048 &    0.045 \\
              &        & PromptSource &            0.584 &           0.780 &          0.735 &        0.041 &    0.044 \\
              &        & Null Instruction &            0.660 &           0.792 &          0.756 &        0.042 &    0.040 \\
              &        & RLPrompt &            0.700 &           0.799 &          0.758 &        0.041 &    0.041 \\
              & gptneo1b3 & APE &            0.520 &           0.605 &          0.511 &        0.062 &    0.065 \\
              &        & Ad hoc &            0.544 &           0.672 &          0.596 &        0.036 &    0.038 \\
              &        & Generic Instruction &            0.492 &           0.674 &          0.595 &        0.037 &    0.037 \\
              &        & Low Perplexity &            0.544 &           0.675 &          0.613 &        0.037 &    0.045 \\
              &        & PromptSource &            0.548 &           0.672 &          0.604 &        0.039 &    0.041 \\
              &        & Null Instruction &            0.480 &           0.661 &          0.587 &        0.039 &    0.039 \\
              &        & RLPrompt &            0.576 &           0.669 &          0.590 &        0.037 &    0.042 \\
              & gptneo2b7 & APE &            0.528 &           0.584 &          0.481 &        0.086 &    0.052 \\
              &        & Ad hoc &            0.580 &           0.680 &          0.567 &        0.053 &    0.056 \\
              &        & Generic Instruction &            0.512 &           0.667 &          0.566 &        0.059 &    0.060 \\
              &        & Low Perplexity &            0.588 &           0.687 &          0.589 &        0.065 &    0.039 \\
              &        & PromptSource &            0.592 &           0.690 &          0.586 &        0.057 &    0.049 \\
              &        & Null Instruction &            0.540 &           0.659 &          0.544 &        0.061 &    0.055 \\
              &        & RLPrompt &            0.584 &           0.674 &          0.576 &        0.050 &    0.057 \\
              & gptneox20b & APE &            0.708 &           0.690 &          0.620 &        0.080 &    0.070 \\
              &        & Ad hoc &            0.660 &           0.762 &          0.717 &        0.058 &    0.036 \\
              &        & Generic Instruction &            0.704 &           0.783 &          0.738 &        0.049 &    0.040 \\
              &        & Low Perplexity &            0.552 &           0.725 &          0.685 &        0.064 &    0.045 \\
              &        & PromptSource &            0.668 &           0.761 &          0.706 &        0.057 &    0.043 \\
              &        & Null Instruction &            0.740 &           0.780 &          0.725 &        0.048 &    0.035 \\
              &        & RLPrompt &            0.752 &           0.779 &          0.741 &        0.044 &    0.039 \\
              & llama13b & APE &            0.500 &           0.796 &          0.732 &        0.038 &    0.031 \\
              &        & Ad hoc &            0.556 &           0.801 &          0.735 &        0.032 &    0.026 \\
              &        & Generic Instruction &            0.544 &           0.825 &          0.791 &        0.015 &    0.019 \\
              &        & Low Perplexity &            0.548 &           0.801 &          0.762 &        0.033 &    0.028 \\
              &        & PromptSource &            0.668 &           0.808 &          0.762 &        0.024 &    0.022 \\
              &        & Null Instruction &            0.440 &           0.831 &          0.801 &        0.018 &    0.016 \\
              &        & RLPrompt &            0.436 &           0.830 &          0.797 &        0.018 &    0.012 \\
              & llama7b & APE &            0.308 &           0.759 &          0.652 &        0.056 &    0.058 \\
              &        & Ad hoc &            0.472 &           0.766 &          0.555 &        0.063 &    0.036 \\
              &        & Generic Instruction &            0.332 &           0.769 &          0.562 &        0.070 &    0.042 \\
              &        & Low Perplexity &            0.628 &           0.759 &          0.561 &        0.048 &    0.039 \\
              &        & PromptSource &            0.572 &           0.777 &          0.608 &        0.052 &    0.037 \\
              &        & Null Instruction &            0.540 &           0.804 &          0.612 &        0.059 &    0.044 \\
              &        & RLPrompt &            0.264 &           0.785 &          0.564 &        0.063 &    0.045 \\
              & opt13b & APE &            0.616 &           0.530 &          0.463 &        0.102 &    0.077 \\
              &        & Ad hoc &            0.656 &           0.632 &          0.578 &        0.102 &    0.083 \\
              &        & Generic Instruction &            0.752 &           0.629 &          0.578 &        0.092 &    0.079 \\
              &        & Low Perplexity &            0.648 &           0.594 &          0.527 &        0.095 &    0.069 \\
              &        & PromptSource &            0.652 &           0.624 &          0.568 &        0.097 &    0.072 \\
              &        & Null Instruction &            0.780 &           0.608 &          0.563 &        0.078 &    0.076 \\
              &        & RLPrompt &            0.696 &           0.638 &          0.591 &        0.098 &    0.069 \\
              & opt1b3 & APE &            0.680 &           0.436 &          0.428 &        0.100 &    0.074 \\
              &        & Ad hoc &            0.680 &           0.565 &          0.511 &        0.127 &    0.121 \\
              &        & Generic Instruction &            0.716 &           0.604 &          0.544 &        0.150 &    0.120 \\
              &        & Low Perplexity &            0.660 &           0.493 &          0.451 &        0.122 &    0.124 \\
              &        & PromptSource &            0.680 &           0.538 &          0.483 &        0.130 &    0.125 \\
              &        & Null Instruction &            0.680 &           0.601 &          0.528 &        0.159 &    0.113 \\
              &        & RLPrompt &            0.700 &           0.618 &          0.531 &        0.150 &    0.129 \\
              & opt2b7 & APE &            0.580 &           0.440 &          0.407 &        0.066 &    0.071 \\
              &        & Ad hoc &            0.644 &           0.596 &          0.522 &        0.085 &    0.073 \\
              &        & Generic Instruction &            0.676 &           0.623 &          0.531 &        0.085 &    0.065 \\
              &        & Low Perplexity &            0.600 &           0.580 &          0.496 &        0.067 &    0.070 \\
              &        & PromptSource &            0.636 &           0.585 &          0.507 &        0.076 &    0.069 \\
              &        & Null Instruction &            0.680 &           0.628 &          0.548 &        0.086 &    0.067 \\
              &        & RLPrompt &            0.684 &           0.619 &          0.537 &        0.088 &    0.080 \\
              & opt6b7 & APE &            0.600 &           0.630 &          0.566 &        0.070 &    0.046 \\
              &        & Ad hoc &            0.620 &           0.709 &          0.664 &        0.046 &    0.041 \\
              &        & Generic Instruction &            0.712 &           0.722 &          0.688 &        0.033 &    0.040 \\
              &        & Low Perplexity &            0.636 &           0.712 &          0.653 &        0.049 &    0.042 \\
              &        & PromptSource &            0.644 &           0.716 &          0.673 &        0.040 &    0.036 \\
              &        & Null Instruction &            0.720 &           0.728 &          0.696 &        0.034 &    0.045 \\
              &        & RLPrompt &            0.772 &           0.734 &          0.695 &        0.033 &    0.036 \\
ANLI & bloom1b1 & APE &            0.336 &           0.343 &          0.343 &        0.032 &    0.025 \\
              &        & Ad hoc &            0.340 &           0.342 &          0.345 &        0.041 &    0.037 \\
              &        & Generic Instruction &            0.340 &           0.342 &          0.341 &        0.044 &    0.037 \\
              &        & Low Perplexity &            0.340 &           0.345 &          0.349 &        0.039 &    0.044 \\
              &        & PromptSource &            0.340 &           0.342 &          0.343 &        0.039 &    0.039 \\
              &        & Null Instruction &            0.340 &           0.344 &          0.340 &        0.039 &    0.039 \\
              &        & RLPrompt &            0.340 &           0.338 &          0.340 &        0.039 &    0.032 \\
              & bloom1b7 & APE &            0.356 &           0.339 &          0.338 &        0.027 &    0.020 \\
              &        & Ad hoc &            0.336 &           0.346 &          0.347 &        0.022 &    0.031 \\
              &        & Generic Instruction &            0.324 &           0.346 &          0.343 &        0.031 &    0.029 \\
              &        & Low Perplexity &            0.332 &           0.344 &          0.347 &        0.016 &    0.029 \\
              &        & PromptSource &            0.328 &           0.348 &          0.346 &        0.025 &    0.031 \\
              &        & Null Instruction &            0.320 &           0.347 &          0.333 &        0.045 &    0.033 \\
              &        & RLPrompt &            0.324 &           0.353 &          0.342 &        0.039 &    0.025 \\
              & bloom3b & APE &            0.336 &           0.345 &          0.345 &        0.051 &    0.041 \\
              &        & Ad hoc &            0.340 &           0.366 &          0.358 &        0.040 &    0.056 \\
              &        & Generic Instruction &            0.348 &           0.375 &          0.354 &        0.053 &    0.043 \\
              &        & Low Perplexity &            0.340 &           0.371 &          0.357 &        0.035 &    0.052 \\
              &        & PromptSource &            0.340 &           0.370 &          0.351 &        0.037 &    0.053 \\
              &        & Null Instruction &            0.380 &           0.355 &          0.341 &        0.044 &    0.036 \\
              &        & RLPrompt &            0.352 &           0.359 &          0.348 &        0.043 &    0.047 \\
              & bloom7b1 & APE &            0.324 &           0.321 &          0.326 &        0.045 &    0.037 \\
              &        & Ad hoc &            0.340 &           0.320 &          0.323 &        0.024 &    0.030 \\
              &        & Generic Instruction &            0.340 &           0.324 &          0.326 &        0.021 &    0.039 \\
              &        & Low Perplexity &            0.340 &           0.319 &          0.329 &        0.023 &    0.027 \\
              &        & PromptSource &            0.340 &           0.323 &          0.328 &        0.019 &    0.027 \\
              &        & Null Instruction &            0.340 &           0.331 &          0.328 &        0.018 &    0.031 \\
              &        & RLPrompt &            0.336 &           0.326 &          0.328 &        0.018 &    0.035 \\
              & gptneo1b3 & APE &            0.344 &           0.354 &          0.338 &        0.036 &    0.024 \\
              &        & Ad hoc &            0.340 &           0.339 &          0.341 &        0.005 &    0.000 \\
              &        & Generic Instruction &            0.340 &           0.339 &          0.340 &        0.005 &    0.000 \\
              &        & Low Perplexity &            0.340 &           0.340 &          0.340 &        0.001 &    0.000 \\
              &        & PromptSource &            0.340 &           0.339 &          0.340 &        0.003 &    0.000 \\
              &        & Null Instruction &            0.340 &           0.339 &          0.340 &        0.005 &    0.000 \\
              &        & RLPrompt &            0.340 &           0.339 &          0.340 &        0.005 &    0.001 \\
              & gptneo2b7 & APE &            0.348 &           0.345 &          0.340 &        0.016 &    0.006 \\
              &        & Ad hoc &            0.340 &           0.340 &          0.340 &        0.000 &    0.000 \\
              &        & Generic Instruction &            0.340 &           0.340 &          0.340 &        0.000 &    0.000 \\
              &        & Low Perplexity &            0.340 &           0.340 &          0.340 &        0.000 &    0.000 \\
              &        & PromptSource &            0.340 &           0.340 &          0.340 &        0.000 &    0.000 \\
              &        & Null Instruction &            0.340 &           0.340 &          0.340 &        0.000 &    0.000 \\
              &        & RLPrompt &            0.340 &           0.340 &          0.340 &        0.000 &    0.000 \\
              & gptneox20b & APE &            0.348 &           0.306 &          0.323 &        0.040 &    0.035 \\
              &        & Ad hoc &            0.340 &           0.309 &          0.340 &        0.042 &    0.040 \\
              &        & Generic Instruction &            0.340 &           0.305 &          0.336 &        0.047 &    0.042 \\
              &        & Low Perplexity &            0.340 &           0.315 &          0.338 &        0.040 &    0.048 \\
              &        & PromptSource &            0.340 &           0.319 &          0.335 &        0.033 &    0.030 \\
              &        & Null Instruction &            0.340 &           0.308 &          0.347 &        0.051 &    0.027 \\
              &        & RLPrompt &            0.340 &           0.313 &          0.341 &        0.042 &    0.035 \\
              & llama13b & APE &            0.328 &           0.359 &          0.357 &        0.044 &    0.030 \\
              &        & Ad hoc &            0.392 &           0.347 &          0.344 &        0.044 &    0.028 \\
              &        & Generic Instruction &            0.396 &           0.346 &          0.342 &        0.032 &    0.024 \\
              &        & Low Perplexity &            0.444 &           0.348 &          0.347 &        0.036 &    0.027 \\
              &        & PromptSource &            0.444 &           0.349 &          0.350 &        0.036 &    0.023 \\
              &        & Null Instruction &            0.360 &           0.356 &          0.351 &        0.035 &    0.020 \\
              &        & RLPrompt &            0.364 &           0.349 &          0.344 &        0.035 &    0.032 \\
              & llama7b & APE &            0.316 &           0.342 &          0.317 &        0.034 &    0.027 \\
              &        & Ad hoc &            0.372 &           0.333 &          0.338 &        0.025 &    0.009 \\
              &        & Generic Instruction &            0.344 &           0.329 &          0.341 &        0.027 &    0.013 \\
              &        & Low Perplexity &            0.376 &           0.335 &          0.338 &        0.018 &    0.002 \\
              &        & PromptSource &            0.388 &           0.334 &          0.335 &        0.019 &    0.004 \\
              &        & Null Instruction &            0.420 &           0.324 &          0.344 &        0.026 &    0.012 \\
              &        & RLPrompt &            0.412 &           0.330 &          0.339 &        0.019 &    0.010 \\
              & opt13b & APE &            0.292 &           0.339 &          0.331 &        0.009 &    0.017 \\
              &        & Ad hoc &            0.340 &           0.338 &          0.342 &        0.007 &    0.007 \\
              &        & Generic Instruction &            0.340 &           0.338 &          0.339 &        0.006 &    0.001 \\
              &        & Low Perplexity &            0.340 &           0.341 &          0.339 &        0.002 &    0.003 \\
              &        & PromptSource &            0.340 &           0.341 &          0.339 &        0.003 &    0.006 \\
              &        & Null Instruction &            0.340 &           0.340 &          0.337 &        0.000 &    0.000 \\
              &        & RLPrompt &            0.340 &           0.340 &          0.339 &        0.000 &    0.001 \\
              & opt1b3 & APE &            0.352 &           0.341 &          0.333 &        0.019 &    0.015 \\
              &        & Ad hoc &            0.340 &           0.329 &          0.329 &        0.022 &    0.015 \\
              &        & Generic Instruction &            0.340 &           0.333 &          0.324 &        0.016 &    0.011 \\
              &        & Low Perplexity &            0.340 &           0.327 &          0.324 &        0.025 &    0.009 \\
              &        & PromptSource &            0.340 &           0.326 &          0.329 &        0.025 &    0.015 \\
              &        & Null Instruction &            0.340 &           0.328 &          0.323 &        0.025 &    0.012 \\
              &        & RLPrompt &            0.340 &           0.330 &          0.322 &        0.024 &    0.008 \\
              & opt2b7 & APE &            0.328 &           0.322 &          0.323 &        0.034 &    0.029 \\
              &        & Ad hoc &            0.340 &           0.344 &          0.349 &        0.022 &    0.037 \\
              &        & Generic Instruction &            0.340 &           0.340 &          0.343 &        0.017 &    0.026 \\
              &        & Low Perplexity &            0.340 &           0.346 &          0.352 &        0.028 &    0.036 \\
              &        & PromptSource &            0.340 &           0.337 &          0.349 &        0.023 &    0.038 \\
              &        & Null Instruction &            0.340 &           0.340 &          0.348 &        0.015 &    0.017 \\
              &        & RLPrompt &            0.340 &           0.339 &          0.344 &        0.019 &    0.029 \\
              & opt6b7 & APE &            0.300 &           0.340 &          0.339 &        0.000 &    0.002 \\
              &        & Ad hoc &            0.340 &           0.334 &          0.335 &        0.020 &    0.017 \\
              &        & Generic Instruction &            0.340 &           0.328 &          0.333 &        0.025 &    0.020 \\
              &        & Low Perplexity &            0.340 &           0.335 &          0.336 &        0.020 &    0.012 \\
              &        & PromptSource &            0.340 &           0.330 &          0.335 &        0.030 &    0.013 \\
              &        & Null Instruction &            0.340 &           0.332 &          0.332 &        0.015 &    0.031 \\
              &        & RLPrompt &            0.340 &           0.335 &          0.340 &        0.021 &    0.013 \\
BoolQ & bloom1b1 & APE &            0.524 &           0.503 &          0.473 &        0.050 &    0.020 \\
              &        & Ad hoc &            0.524 &           0.510 &          0.469 &        0.051 &    0.029 \\
              &        & Generic Instruction &            0.520 &           0.506 &          0.461 &        0.056 &    0.032 \\
              &        & Low Perplexity &            0.540 &           0.516 &          0.484 &        0.052 &    0.031 \\
              &        & PromptSource &            0.512 &           0.505 &          0.480 &        0.051 &    0.022 \\
              &        & Null Instruction &            0.500 &           0.511 &          0.449 &        0.047 &    0.033 \\
              &        & RLPrompt &            0.504 &           0.505 &          0.448 &        0.048 &    0.035 \\
              & bloom1b7 & APE &            0.424 &           0.419 &          0.435 &        0.050 &    0.027 \\
              &        & Ad hoc &            0.436 &           0.418 &          0.432 &        0.049 &    0.024 \\
              &        & Generic Instruction &            0.428 &           0.415 &          0.422 &        0.046 &    0.021 \\
              &        & Low Perplexity &            0.416 &           0.418 &          0.435 &        0.046 &    0.021 \\
              &        & PromptSource &            0.420 &           0.413 &          0.432 &        0.049 &    0.023 \\
              &        & Null Instruction &            0.460 &           0.425 &          0.424 &        0.042 &    0.029 \\
              &        & RLPrompt &            0.456 &           0.417 &          0.425 &        0.043 &    0.018 \\
              & bloom3b & APE &            0.484 &           0.463 &          0.439 &        0.045 &    0.031 \\
              &        & Ad hoc &            0.492 &           0.469 &          0.434 &        0.049 &    0.034 \\
              &        & Generic Instruction &            0.496 &           0.466 &          0.446 &        0.048 &    0.044 \\
              &        & Low Perplexity &            0.500 &           0.451 &          0.430 &        0.043 &    0.033 \\
              &        & PromptSource &            0.496 &           0.460 &          0.442 &        0.049 &    0.041 \\
              &        & Null Instruction &            0.500 &           0.476 &          0.455 &        0.044 &    0.041 \\
              &        & RLPrompt &            0.492 &           0.466 &          0.455 &        0.053 &    0.041 \\
              & bloom7b1 & APE &            0.488 &           0.535 &          0.508 &        0.063 &    0.049 \\
              &        & Ad hoc &            0.480 &           0.538 &          0.500 &        0.062 &    0.053 \\
              &        & Generic Instruction &            0.476 &           0.545 &          0.512 &        0.060 &    0.045 \\
              &        & Low Perplexity &            0.476 &           0.531 &          0.501 &        0.058 &    0.050 \\
              &        & PromptSource &            0.492 &           0.517 &          0.499 &        0.069 &    0.046 \\
              &        & Null Instruction &            0.520 &           0.555 &          0.520 &        0.056 &    0.041 \\
              &        & RLPrompt &            0.456 &           0.547 &          0.521 &        0.050 &    0.044 \\
              & gptneo1b3 & APE &            0.536 &           0.557 &          0.575 &        0.052 &    0.045 \\
              &        & Ad hoc &            0.536 &           0.548 &          0.576 &        0.046 &    0.041 \\
              &        & Generic Instruction &            0.556 &           0.549 &          0.573 &        0.055 &    0.045 \\
              &        & Low Perplexity &            0.524 &           0.549 &          0.577 &        0.046 &    0.032 \\
              &        & PromptSource &            0.528 &           0.554 &          0.580 &        0.047 &    0.047 \\
              &        & Null Instruction &            0.540 &           0.545 &          0.559 &        0.057 &    0.035 \\
              &        & RLPrompt &            0.520 &           0.553 &          0.566 &        0.052 &    0.047 \\
              & gptneo2b7 & APE &            0.484 &           0.506 &          0.510 &        0.044 &    0.036 \\
              &        & Ad hoc &            0.504 &           0.504 &          0.497 &        0.043 &    0.035 \\
              &        & Generic Instruction &            0.512 &           0.494 &          0.506 &        0.046 &    0.027 \\
              &        & Low Perplexity &            0.468 &           0.505 &          0.493 &        0.042 &    0.037 \\
              &        & PromptSource &            0.484 &           0.517 &          0.514 &        0.041 &    0.031 \\
              &        & Null Instruction &            0.500 &           0.500 &          0.507 &        0.052 &    0.031 \\
              &        & RLPrompt &            0.508 &           0.495 &          0.505 &        0.050 &    0.023 \\
              & gptneox20b & APE &            0.564 &           0.616 &          0.615 &        0.058 &    0.054 \\
              &        & Ad hoc &            0.580 &           0.619 &          0.611 &        0.054 &    0.053 \\
              &        & Generic Instruction &            0.592 &           0.626 &          0.616 &        0.065 &    0.056 \\
              &        & Low Perplexity &            0.508 &           0.617 &          0.618 &        0.055 &    0.062 \\
              &        & PromptSource &            0.560 &           0.607 &          0.618 &        0.063 &    0.051 \\
              &        & Null Instruction &            0.540 &           0.628 &          0.612 &        0.058 &    0.047 \\
              &        & RLPrompt &            0.536 &           0.626 &          0.623 &        0.053 &    0.048 \\
              & llama13b & APE &            0.556 &           0.822 &          0.789 &        0.060 &    0.038 \\
              &        & Ad hoc &            0.556 &           0.807 &          0.774 &        0.067 &    0.041 \\
              &        & Generic Instruction &            0.536 &           0.816 &          0.776 &        0.060 &    0.034 \\
              &        & Low Perplexity &            0.560 &           0.808 &          0.775 &        0.067 &    0.039 \\
              &        & PromptSource &            0.524 &           0.814 &          0.783 &        0.062 &    0.034 \\
              &        & Null Instruction &            0.560 &           0.824 &          0.791 &        0.038 &    0.044 \\
              &        & RLPrompt &            0.540 &           0.819 &          0.781 &        0.051 &    0.046 \\
              & llama7b & APE &            0.532 &           0.743 &          0.719 &        0.036 &    0.041 \\
              &        & Ad hoc &            0.524 &           0.741 &          0.722 &        0.038 &    0.039 \\
              &        & Generic Instruction &            0.540 &           0.751 &          0.739 &        0.039 &    0.039 \\
              &        & Low Perplexity &            0.656 &           0.744 &          0.725 &        0.035 &    0.035 \\
              &        & PromptSource &            0.608 &           0.734 &          0.719 &        0.046 &    0.036 \\
              &        & Null Instruction &            0.580 &           0.757 &          0.744 &        0.058 &    0.044 \\
              &        & RLPrompt &            0.528 &           0.741 &          0.736 &        0.059 &    0.040 \\
              & opt13b & APE &            0.524 &           0.609 &          0.574 &        0.042 &    0.037 \\
              &        & Ad hoc &            0.556 &           0.603 &          0.583 &        0.044 &    0.036 \\
              &        & Generic Instruction &            0.540 &           0.610 &          0.572 &        0.045 &    0.048 \\
              &        & Low Perplexity &            0.552 &           0.599 &          0.585 &        0.057 &    0.024 \\
              &        & PromptSource &            0.576 &           0.595 &          0.563 &        0.045 &    0.030 \\
              &        & Null Instruction &            0.580 &           0.615 &          0.572 &        0.049 &    0.035 \\
              &        & RLPrompt &            0.512 &           0.620 &          0.584 &        0.048 &    0.045 \\
              & opt1b3 & APE &            0.540 &           0.519 &          0.515 &        0.029 &    0.039 \\
              &        & Ad hoc &            0.540 &           0.519 &          0.514 &        0.030 &    0.036 \\
              &        & Generic Instruction &            0.556 &           0.514 &          0.513 &        0.025 &    0.035 \\
              &        & Low Perplexity &            0.512 &           0.520 &          0.512 &        0.032 &    0.033 \\
              &        & PromptSource &            0.508 &           0.514 &          0.513 &        0.026 &    0.039 \\
              &        & Null Instruction &            0.580 &           0.511 &          0.512 &        0.025 &    0.038 \\
              &        & RLPrompt &            0.556 &           0.511 &          0.510 &        0.022 &    0.032 \\
              & opt2b7 & APE &            0.500 &           0.548 &          0.541 &        0.039 &    0.029 \\
              &        & Ad hoc &            0.548 &           0.547 &          0.536 &        0.039 &    0.035 \\
              &        & Generic Instruction &            0.480 &           0.541 &          0.538 &        0.042 &    0.040 \\
              &        & Low Perplexity &            0.552 &           0.548 &          0.531 &        0.039 &    0.029 \\
              &        & PromptSource &            0.540 &           0.545 &          0.533 &        0.041 &    0.036 \\
              &        & Null Instruction &            0.540 &           0.555 &          0.553 &        0.050 &    0.038 \\
              &        & RLPrompt &            0.484 &           0.566 &          0.557 &        0.054 &    0.037 \\
              & opt6b7 & APE &            0.548 &           0.585 &          0.628 &        0.033 &    0.032 \\
              &        & Ad hoc &            0.536 &           0.587 &          0.631 &        0.028 &    0.032 \\
              &        & Generic Instruction &            0.548 &           0.581 &          0.621 &        0.031 &    0.040 \\
              &        & Low Perplexity &            0.560 &           0.582 &          0.630 &        0.036 &    0.030 \\
              &        & PromptSource &            0.488 &           0.583 &          0.623 &        0.041 &    0.030 \\
              &        & Null Instruction &            0.540 &           0.583 &          0.620 &        0.040 &    0.040 \\
              &        & RLPrompt &            0.548 &           0.582 &          0.614 &        0.040 &    0.041 \\
CosmosQA & bloom1b1 & APE &            0.312 &           0.249 &          0.245 &        0.060 &    0.018 \\
              &        & Ad hoc &            0.300 &           0.245 &          0.243 &        0.062 &    0.017 \\
              &        & Generic Instruction &            0.300 &           0.246 &          0.242 &        0.061 &    0.017 \\
              &        & Low Perplexity &            0.300 &           0.244 &          0.242 &        0.060 &    0.019 \\
              &        & PromptSource &            0.292 &           0.242 &          0.242 &        0.062 &    0.016 \\
              &        & Null Instruction &            0.280 &           0.252 &          0.245 &        0.057 &    0.017 \\
              &        & RLPrompt &            0.312 &           0.252 &          0.246 &        0.057 &    0.017 \\
              & bloom1b7 & APE &            0.280 &           0.245 &          0.255 &        0.063 &    0.011 \\
              &        & Ad hoc &            0.260 &           0.241 &          0.253 &        0.065 &    0.008 \\
              &        & Generic Instruction &            0.280 &           0.242 &          0.253 &        0.066 &    0.008 \\
              &        & Low Perplexity &            0.260 &           0.241 &          0.254 &        0.064 &    0.008 \\
              &        & PromptSource &            0.268 &           0.241 &          0.255 &        0.064 &    0.008 \\
              &        & Null Instruction &            0.300 &           0.247 &          0.255 &        0.068 &    0.010 \\
              &        & RLPrompt &            0.284 &           0.245 &          0.255 &        0.068 &    0.009 \\
              & bloom3b & APE &            0.324 &           0.225 &          0.223 &        0.061 &    0.012 \\
              &        & Ad hoc &            0.336 &           0.222 &          0.222 &        0.063 &    0.012 \\
              &        & Generic Instruction &            0.316 &           0.222 &          0.223 &        0.064 &    0.012 \\
              &        & Low Perplexity &            0.324 &           0.224 &          0.221 &        0.062 &    0.011 \\
              &        & PromptSource &            0.312 &           0.222 &          0.224 &        0.064 &    0.010 \\
              &        & Null Instruction &            0.320 &           0.228 &          0.227 &        0.057 &    0.010 \\
              &        & RLPrompt &            0.324 &           0.227 &          0.224 &        0.061 &    0.014 \\
              & bloom7b1 & APE &            0.340 &           0.273 &          0.260 &        0.058 &    0.018 \\
              &        & Ad hoc &            0.320 &           0.270 &          0.260 &        0.059 &    0.014 \\
              &        & Generic Instruction &            0.300 &           0.274 &          0.262 &        0.060 &    0.016 \\
              &        & Low Perplexity &            0.324 &           0.269 &          0.261 &        0.062 &    0.015 \\
              &        & PromptSource &            0.324 &           0.267 &          0.260 &        0.063 &    0.017 \\
              &        & Null Instruction &            0.360 &           0.281 &          0.264 &        0.053 &    0.022 \\
              &        & RLPrompt &            0.348 &           0.275 &          0.261 &        0.058 &    0.015 \\
              & gptneo1b3 & APE &            0.272 &           0.259 &          0.277 &        0.085 &    0.015 \\
              &        & Ad hoc &            0.304 &           0.259 &          0.277 &        0.084 &    0.015 \\
              &        & Generic Instruction &            0.292 &           0.264 &          0.278 &        0.082 &    0.014 \\
              &        & Low Perplexity &            0.296 &           0.261 &          0.279 &        0.083 &    0.014 \\
              &        & PromptSource &            0.284 &           0.259 &          0.278 &        0.086 &    0.013 \\
              &        & Null Instruction &            0.300 &           0.264 &          0.285 &        0.085 &    0.017 \\
              &        & RLPrompt &            0.292 &           0.259 &          0.275 &        0.082 &    0.014 \\
              & gptneo2b7 & APE &            0.324 &           0.222 &          0.273 &        0.078 &    0.014 \\
              &        & Ad hoc &            0.320 &           0.222 &          0.270 &        0.079 &    0.014 \\
              &        & Generic Instruction &            0.336 &           0.223 &          0.272 &        0.078 &    0.017 \\
              &        & Low Perplexity &            0.340 &           0.222 &          0.269 &        0.079 &    0.015 \\
              &        & PromptSource &            0.324 &           0.222 &          0.270 &        0.079 &    0.017 \\
              &        & Null Instruction &            0.340 &           0.224 &          0.273 &        0.075 &    0.018 \\
              &        & RLPrompt &            0.348 &           0.225 &          0.273 &        0.078 &    0.014 \\
              & gptneox20b & APE &            0.356 &           0.333 &          0.335 &        0.098 &    0.016 \\
              &        & Ad hoc &            0.352 &           0.337 &          0.328 &        0.100 &    0.019 \\
              &        & Generic Instruction &            0.344 &           0.337 &          0.330 &        0.097 &    0.017 \\
              &        & Low Perplexity &            0.364 &           0.337 &          0.327 &        0.101 &    0.018 \\
              &        & PromptSource &            0.356 &           0.336 &          0.328 &        0.102 &    0.017 \\
              &        & Null Instruction &            0.360 &           0.335 &          0.331 &        0.092 &    0.020 \\
              &        & RLPrompt &            0.340 &           0.331 &          0.332 &        0.097 &    0.018 \\
              & llama13b & APE &            0.352 &           0.361 &          0.358 &        0.095 &    0.016 \\
              &        & Ad hoc &            0.308 &           0.350 &          0.352 &        0.099 &    0.020 \\
              &        & Generic Instruction &            0.336 &           0.354 &          0.356 &        0.096 &    0.017 \\
              &        & Low Perplexity &            0.300 &           0.353 &          0.352 &        0.104 &    0.019 \\
              &        & PromptSource &            0.308 &           0.351 &          0.350 &        0.100 &    0.020 \\
              &        & Null Instruction &            0.440 &           0.361 &          0.353 &        0.098 &    0.021 \\
              &        & RLPrompt &            0.380 &           0.364 &          0.356 &        0.093 &    0.019 \\
              & llama7b & APE &            0.360 &           0.391 &          0.373 &        0.105 &    0.022 \\
              &        & Ad hoc &            0.344 &           0.389 &          0.367 &        0.100 &    0.019 \\
              &        & Generic Instruction &            0.336 &           0.390 &          0.373 &        0.103 &    0.018 \\
              &        & Low Perplexity &            0.328 &           0.385 &          0.364 &        0.102 &    0.018 \\
              &        & PromptSource &            0.340 &           0.387 &          0.367 &        0.099 &    0.017 \\
              &        & Null Instruction &            0.360 &           0.393 &          0.376 &        0.107 &    0.021 \\
              &        & RLPrompt &            0.360 &           0.393 &          0.379 &        0.103 &    0.020 \\
              & opt13b & APE &            0.352 &           0.355 &          0.322 &        0.109 &    0.026 \\
              &        & Ad hoc &            0.348 &           0.351 &          0.319 &        0.112 &    0.020 \\
              &        & Generic Instruction &            0.356 &           0.352 &          0.322 &        0.112 &    0.022 \\
              &        & Low Perplexity &            0.348 &           0.350 &          0.322 &        0.115 &    0.023 \\
              &        & PromptSource &            0.348 &           0.352 &          0.322 &        0.111 &    0.025 \\
              &        & Null Instruction &            0.420 &           0.365 &          0.332 &        0.114 &    0.026 \\
              &        & RLPrompt &            0.404 &           0.359 &          0.328 &        0.113 &    0.024 \\
              & opt1b3 & APE &            0.312 &           0.260 &          0.261 &        0.077 &    0.014 \\
              &        & Ad hoc &            0.292 &           0.257 &          0.261 &        0.076 &    0.011 \\
              &        & Generic Instruction &            0.320 &           0.257 &          0.261 &        0.075 &    0.012 \\
              &        & Low Perplexity &            0.316 &           0.255 &          0.261 &        0.075 &    0.012 \\
              &        & PromptSource &            0.304 &           0.254 &          0.260 &        0.074 &    0.010 \\
              &        & Null Instruction &            0.320 &           0.257 &          0.268 &        0.077 &    0.014 \\
              &        & RLPrompt &            0.344 &           0.262 &          0.264 &        0.082 &    0.011 \\
              & opt2b7 & APE &            0.352 &           0.283 &          0.310 &        0.079 &    0.027 \\
              &        & Ad hoc &            0.344 &           0.282 &          0.309 &        0.077 &    0.029 \\
              &        & Generic Instruction &            0.348 &           0.284 &          0.311 &        0.078 &    0.027 \\
              &        & Low Perplexity &            0.340 &           0.281 &          0.306 &        0.076 &    0.030 \\
              &        & PromptSource &            0.344 &           0.282 &          0.309 &        0.078 &    0.028 \\
              &        & Null Instruction &            0.360 &           0.292 &          0.315 &        0.077 &    0.024 \\
              &        & RLPrompt &            0.336 &           0.288 &          0.314 &        0.080 &    0.021 \\
              & opt6b7 & APE &            0.340 &           0.337 &          0.373 &        0.091 &    0.021 \\
              &        & Ad hoc &            0.340 &           0.338 &          0.369 &        0.090 &    0.018 \\
              &        & Generic Instruction &            0.336 &           0.334 &          0.369 &        0.089 &    0.020 \\
              &        & Low Perplexity &            0.340 &           0.341 &          0.368 &        0.092 &    0.018 \\
              &        & PromptSource &            0.324 &           0.336 &          0.368 &        0.091 &    0.020 \\
              &        & Null Instruction &            0.380 &           0.335 &          0.372 &        0.092 &    0.023 \\
              &        & RLPrompt &            0.368 &           0.334 &          0.368 &        0.091 &    0.017 \\
HellaSwag & bloom1b1 & APE &            0.412 &           0.397 &          0.375 &        0.026 &    0.009 \\
              &        & Ad hoc &            0.400 &           0.394 &          0.374 &        0.027 &    0.008 \\
              &        & Generic Instruction &            0.424 &           0.395 &          0.375 &        0.028 &    0.008 \\
              &        & Low Perplexity &            0.396 &           0.393 &          0.374 &        0.027 &    0.008 \\
              &        & PromptSource &            0.376 &           0.393 &          0.375 &        0.028 &    0.007 \\
              &        & Null Instruction &            0.420 &           0.396 &          0.377 &        0.027 &    0.010 \\
              &        & RLPrompt &            0.436 &           0.397 &          0.378 &        0.026 &    0.009 \\
              & bloom1b7 & APE &            0.464 &           0.410 &          0.412 &        0.032 &    0.010 \\
              &        & Ad hoc &            0.460 &           0.408 &          0.415 &        0.034 &    0.012 \\
              &        & Generic Instruction &            0.460 &           0.411 &          0.414 &        0.032 &    0.012 \\
              &        & Low Perplexity &            0.456 &           0.409 &          0.417 &        0.031 &    0.012 \\
              &        & PromptSource &            0.456 &           0.410 &          0.417 &        0.031 &    0.012 \\
              &        & Null Instruction &            0.480 &           0.408 &          0.412 &        0.032 &    0.014 \\
              &        & RLPrompt &            0.464 &           0.409 &          0.414 &        0.032 &    0.013 \\
              & bloom3b & APE &            0.456 &           0.481 &          0.467 &        0.023 &    0.014 \\
              &        & Ad hoc &            0.456 &           0.481 &          0.467 &        0.024 &    0.014 \\
              &        & Generic Instruction &            0.468 &           0.479 &          0.467 &        0.024 &    0.014 \\
              &        & Low Perplexity &            0.448 &           0.482 &          0.467 &        0.025 &    0.014 \\
              &        & PromptSource &            0.464 &           0.479 &          0.468 &        0.025 &    0.013 \\
              &        & Null Instruction &            0.480 &           0.484 &          0.469 &        0.023 &    0.013 \\
              &        & RLPrompt &            0.480 &           0.483 &          0.470 &        0.022 &    0.012 \\
              & bloom7b1 & APE &            0.540 &           0.561 &          0.542 &        0.018 &    0.013 \\
              &        & Ad hoc &            0.552 &           0.561 &          0.544 &        0.018 &    0.011 \\
              &        & Generic Instruction &            0.528 &           0.560 &          0.544 &        0.021 &    0.013 \\
              &        & Low Perplexity &            0.540 &           0.561 &          0.544 &        0.017 &    0.011 \\
              &        & PromptSource &            0.536 &           0.560 &          0.544 &        0.019 &    0.013 \\
              &        & Null Instruction &            0.600 &           0.563 &          0.543 &        0.018 &    0.012 \\
              &        & RLPrompt &            0.564 &           0.566 &          0.543 &        0.017 &    0.014 \\
              & gptneo1b3 & APE &            0.420 &           0.402 &          0.411 &        0.019 &    0.011 \\
              &        & Ad hoc &            0.440 &           0.401 &          0.409 &        0.018 &    0.010 \\
              &        & Generic Instruction &            0.448 &           0.402 &          0.409 &        0.017 &    0.010 \\
              &        & Low Perplexity &            0.428 &           0.400 &          0.409 &        0.018 &    0.009 \\
              &        & PromptSource &            0.436 &           0.401 &          0.411 &        0.018 &    0.010 \\
              &        & Null Instruction &            0.420 &           0.401 &          0.408 &        0.018 &    0.011 \\
              &        & RLPrompt &            0.436 &           0.407 &          0.408 &        0.015 &    0.009 \\
              & gptneo2b7 & APE &            0.452 &           0.483 &          0.470 &        0.024 &    0.008 \\
              &        & Ad hoc &            0.452 &           0.481 &          0.469 &        0.025 &    0.008 \\
              &        & Generic Instruction &            0.452 &           0.481 &          0.470 &        0.026 &    0.007 \\
              &        & Low Perplexity &            0.444 &           0.481 &          0.470 &        0.025 &    0.009 \\
              &        & PromptSource &            0.452 &           0.482 &          0.470 &        0.024 &    0.008 \\
              &        & Null Instruction &            0.460 &           0.484 &          0.472 &        0.024 &    0.007 \\
              &        & RLPrompt &            0.464 &           0.486 &          0.472 &        0.024 &    0.009 \\
              & gptneox20b & APE &            0.584 &           0.641 &          0.612 &        0.030 &    0.010 \\
              &        & Ad hoc &            0.596 &           0.643 &          0.612 &        0.031 &    0.012 \\
              &        & Generic Instruction &            0.568 &           0.644 &          0.611 &        0.033 &    0.009 \\
              &        & Low Perplexity &            0.580 &           0.642 &          0.613 &        0.031 &    0.012 \\
              &        & PromptSource &            0.584 &           0.643 &          0.613 &        0.031 &    0.006 \\
              &        & Null Instruction &            0.600 &           0.644 &          0.616 &        0.033 &    0.010 \\
              &        & RLPrompt &            0.580 &           0.642 &          0.617 &        0.029 &    0.009 \\
              & llama13b & APE &            0.764 &           0.765 &          0.771 &        0.024 &    0.010 \\
              &        & Ad hoc &            0.796 &           0.763 &          0.770 &        0.022 &    0.010 \\
              &        & Generic Instruction &            0.792 &           0.769 &          0.770 &        0.026 &    0.012 \\
              &        & Low Perplexity &            0.780 &           0.763 &          0.769 &        0.023 &    0.012 \\
              &        & PromptSource &            0.780 &           0.764 &          0.771 &        0.023 &    0.012 \\
              &        & Null Instruction &            0.800 &           0.769 &          0.768 &        0.026 &    0.009 \\
              &        & RLPrompt &            0.796 &           0.766 &          0.769 &        0.022 &    0.009 \\
              & llama7b & APE &            0.632 &           0.742 &          0.715 &        0.019 &    0.012 \\
              &        & Ad hoc &            0.644 &           0.742 &          0.716 &        0.018 &    0.014 \\
              &        & Generic Instruction &            0.632 &           0.741 &          0.715 &        0.018 &    0.012 \\
              &        & Low Perplexity &            0.652 &           0.743 &          0.716 &        0.018 &    0.014 \\
              &        & PromptSource &            0.640 &           0.741 &          0.714 &        0.019 &    0.013 \\
              &        & Null Instruction &            0.680 &           0.744 &          0.720 &        0.019 &    0.013 \\
              &        & RLPrompt &            0.676 &           0.743 &          0.718 &        0.019 &    0.011 \\
              & opt13b & APE &            0.616 &           0.638 &          0.602 &        0.043 &    0.015 \\
              &        & Ad hoc &            0.620 &           0.632 &          0.605 &        0.038 &    0.018 \\
              &        & Generic Instruction &            0.612 &           0.634 &          0.603 &        0.041 &    0.019 \\
              &        & Low Perplexity &            0.616 &           0.631 &          0.603 &        0.038 &    0.018 \\
              &        & PromptSource &            0.612 &           0.633 &          0.600 &        0.040 &    0.017 \\
              &        & Null Instruction &            0.620 &           0.639 &          0.604 &        0.044 &    0.018 \\
              &        & RLPrompt &            0.616 &           0.637 &          0.605 &        0.041 &    0.016 \\
              & opt1b3 & APE &            0.512 &           0.500 &          0.484 &        0.014 &    0.006 \\
              &        & Ad hoc &            0.516 &           0.501 &          0.487 &        0.015 &    0.007 \\
              &        & Generic Instruction &            0.520 &           0.501 &          0.489 &        0.014 &    0.008 \\
              &        & Low Perplexity &            0.516 &           0.501 &          0.487 &        0.015 &    0.007 \\
              &        & PromptSource &            0.504 &           0.501 &          0.489 &        0.014 &    0.007 \\
              &        & Null Instruction &            0.520 &           0.501 &          0.489 &        0.014 &    0.005 \\
              &        & RLPrompt &            0.524 &           0.501 &          0.489 &        0.013 &    0.006 \\
              & opt2b7 & APE &            0.524 &           0.532 &          0.539 &        0.023 &    0.013 \\
              &        & Ad hoc &            0.520 &           0.530 &          0.539 &        0.023 &    0.009 \\
              &        & Generic Instruction &            0.520 &           0.532 &          0.541 &        0.025 &    0.012 \\
              &        & Low Perplexity &            0.520 &           0.529 &          0.537 &        0.025 &    0.007 \\
              &        & PromptSource &            0.520 &           0.531 &          0.539 &        0.023 &    0.010 \\
              &        & Null Instruction &            0.540 &           0.533 &          0.540 &        0.024 &    0.011 \\
              &        & RLPrompt &            0.524 &           0.533 &          0.540 &        0.023 &    0.012 \\
              & opt6b7 & APE &            0.560 &           0.568 &          0.561 &        0.021 &    0.012 \\
              &        & Ad hoc &            0.552 &           0.568 &          0.560 &        0.023 &    0.011 \\
              &        & Generic Instruction &            0.572 &           0.573 &          0.561 &        0.019 &    0.012 \\
              &        & Low Perplexity &            0.552 &           0.570 &          0.561 &        0.021 &    0.013 \\
              &        & PromptSource &            0.556 &           0.575 &          0.564 &        0.022 &    0.012 \\
              &        & Null Instruction &            0.580 &           0.567 &          0.561 &        0.018 &    0.014 \\
              &        & RLPrompt &            0.580 &           0.566 &          0.558 &        0.023 &    0.011 \\
IMDB & bloom1b1 & APE &            0.648 &           0.571 &          0.520 &        0.107 &    0.077 \\
              &        & Ad hoc &            0.720 &           0.604 &          0.551 &        0.095 &    0.090 \\
              &        & Generic Instruction &            0.676 &           0.599 &          0.553 &        0.093 &    0.063 \\
              &        & Low Perplexity &            0.728 &           0.589 &          0.529 &        0.107 &    0.089 \\
              &        & PromptSource &            0.744 &           0.587 &          0.541 &        0.096 &    0.084 \\
              &        & Null Instruction &            0.560 &           0.563 &          0.553 &        0.094 &    0.052 \\
              &        & RLPrompt &            0.660 &           0.606 &          0.553 &        0.091 &    0.093 \\
              & bloom1b7 & APE &            0.748 &           0.671 &          0.600 &        0.124 &    0.102 \\
              &        & Ad hoc &            0.688 &           0.712 &          0.628 &        0.101 &    0.095 \\
              &        & Generic Instruction &            0.740 &           0.701 &          0.621 &        0.120 &    0.106 \\
              &        & Low Perplexity &            0.652 &           0.707 &          0.629 &        0.105 &    0.100 \\
              &        & PromptSource &            0.740 &           0.700 &          0.622 &        0.106 &    0.104 \\
              &        & Null Instruction &            0.680 &           0.663 &          0.589 &        0.127 &    0.099 \\
              &        & RLPrompt &            0.712 &           0.687 &          0.617 &        0.117 &    0.102 \\
              & bloom3b & APE &            0.696 &           0.507 &          0.501 &        0.020 &    0.005 \\
              &        & Ad hoc &            0.752 &           0.510 &          0.503 &        0.031 &    0.007 \\
              &        & Generic Instruction &            0.724 &           0.511 &          0.502 &        0.029 &    0.008 \\
              &        & Low Perplexity &            0.684 &           0.509 &          0.502 &        0.026 &    0.003 \\
              &        & PromptSource &            0.768 &           0.510 &          0.503 &        0.027 &    0.007 \\
              &        & Null Instruction &            0.700 &           0.501 &          0.500 &        0.005 &    0.003 \\
              &        & RLPrompt &            0.664 &           0.504 &          0.501 &        0.017 &    0.001 \\
              & bloom7b1 & APE &            0.688 &           0.734 &          0.678 &        0.084 &    0.093 \\
              &        & Ad hoc &            0.824 &           0.763 &          0.705 &        0.078 &    0.065 \\
              &        & Generic Instruction &            0.776 &           0.757 &          0.713 &        0.074 &    0.078 \\
              &        & Low Perplexity &            0.704 &           0.751 &          0.690 &        0.080 &    0.071 \\
              &        & PromptSource &            0.788 &           0.755 &          0.705 &        0.077 &    0.072 \\
              &        & Null Instruction &            0.680 &           0.721 &          0.652 &        0.078 &      0.000 \\
              &        & RLPrompt &            0.676 &           0.745 &          0.694 &        0.083 &    0.092 \\
              & gptneo1b3 & APE &            0.708 &           0.785 &          0.760 &        0.052 &    0.026 \\
              &        & Ad hoc &            0.684 &           0.788 &          0.755 &        0.048 &    0.027 \\
              &        & Generic Instruction &            0.684 &           0.789 &          0.765 &        0.044 &    0.024 \\
              &        & Low Perplexity &            0.692 &           0.783 &          0.757 &        0.051 &    0.025 \\
              &        & PromptSource &            0.724 &           0.787 &          0.756 &        0.048 &    0.031 \\
              &        & Null Instruction &            0.620 &           0.783 &          0.764 &        0.058 &    0.024 \\
              &        & RLPrompt &            0.656 &           0.788 &          0.765 &        0.047 &    0.028 \\
              & gptneo2b7 & APE &            0.800 &           0.777 &          0.715 &        0.088 &    0.096 \\
              &        & Ad hoc &            0.820 &           0.774 &          0.713 &        0.087 &    0.095 \\
              &        & Generic Instruction &            0.816 &           0.782 &          0.727 &        0.080 &    0.086 \\
              &        & Low Perplexity &            0.836 &           0.772 &          0.702 &        0.097 &    0.096 \\
              &        & PromptSource &            0.816 &           0.787 &          0.727 &        0.088 &    0.090 \\
              &        & Null Instruction &            0.800 &           0.793 &          0.739 &        0.072 &    0.081 \\
              &        & RLPrompt &            0.800 &           0.770 &          0.714 &        0.090 &    0.086 \\
              & gptneox20b & APE &            0.832 &           0.910 &          0.893 &        0.020 &    0.014 \\
              &        & Ad hoc &            0.872 &           0.909 &          0.893 &        0.018 &    0.017 \\
              &        & Generic Instruction &            0.880 &           0.912 &          0.890 &        0.018 &    0.018 \\
              &        & Low Perplexity &            0.888 &           0.911 &          0.896 &        0.020 &    0.014 \\
              &        & PromptSource &            0.864 &           0.907 &          0.895 &        0.020 &    0.014 \\
              &        & Null Instruction &            0.880 &           0.912 &          0.895 &        0.018 &    0.020 \\
              &        & RLPrompt &            0.860 &           0.912 &          0.898 &        0.018 &    0.017 \\
              & llama13b & APE &            0.660 &           0.900 &          0.905 &        0.026 &    0.033 \\
              &        & Ad hoc &            0.632 &           0.909 &          0.916 &        0.022 &    0.017 \\
              &        & Generic Instruction &            0.628 &           0.908 &          0.917 &        0.024 &    0.018 \\
              &        & Low Perplexity &            0.716 &           0.902 &          0.909 &        0.026 &    0.021 \\
              &        & PromptSource &            0.684 &           0.906 &          0.913 &        0.023 &    0.020 \\
              &        & Null Instruction &            0.580 &           0.908 &          0.919 &        0.020 &    0.013 \\
              &        & RLPrompt &            0.624 &           0.907 &          0.915 &        0.023 &    0.021 \\
              & llama7b & APE &            0.640 &           0.890 &          0.868 &        0.059 &    0.065 \\
              &        & Ad hoc &            0.712 &           0.893 &          0.882 &        0.061 &    0.068 \\
              &        & Generic Instruction &            0.716 &           0.899 &          0.882 &        0.056 &    0.069 \\
              &        & Low Perplexity &            0.752 &           0.898 &          0.878 &        0.060 &    0.063 \\
              &        & PromptSource &            0.728 &           0.899 &          0.879 &        0.059 &    0.067 \\
              &        & Null Instruction &            0.780 &           0.897 &          0.891 &        0.065 &    0.068 \\
              &        & RLPrompt &            0.688 &           0.895 &          0.888 &        0.058 &    0.065 \\
              & opt13b & APE &            0.620 &           0.897 &          0.903 &        0.032 &    0.029 \\
              &        & Ad hoc &            0.668 &           0.905 &          0.903 &        0.023 &    0.023 \\
              &        & Generic Instruction &            0.696 &           0.899 &          0.903 &        0.029 &    0.026 \\
              &        & Low Perplexity &            0.652 &           0.903 &          0.903 &        0.027 &    0.023 \\
              &        & PromptSource &            0.684 &           0.903 &          0.904 &        0.024 &    0.024 \\
              &        & Null Instruction &            0.680 &           0.911 &          0.903 &        0.017 &    0.026 \\
              &        & RLPrompt &            0.696 &           0.899 &          0.903 &        0.030 &    0.027 \\
              & opt1b3 & APE &            0.708 &           0.815 &          0.827 &        0.062 &    0.032 \\
              &        & Ad hoc &            0.736 &           0.806 &          0.815 &        0.069 &    0.036 \\
              &        & Generic Instruction &            0.732 &           0.806 &          0.819 &        0.068 &    0.036 \\
              &        & Low Perplexity &            0.712 &           0.806 &          0.818 &        0.068 &    0.036 \\
              &        & PromptSource &            0.716 &           0.808 &          0.816 &        0.063 &    0.035 \\
              &        & Null Instruction &            0.700 &           0.807 &          0.823 &        0.062 &    0.048 \\
              &        & RLPrompt &            0.700 &           0.793 &          0.805 &        0.074 &    0.045 \\
              & opt2b7 & APE &            0.768 &           0.843 &          0.814 &        0.033 &    0.033 \\
              &        & Ad hoc &            0.700 &           0.848 &          0.819 &        0.039 &    0.034 \\
              &        & Generic Instruction &            0.752 &           0.845 &          0.813 &        0.036 &    0.034 \\
              &        & Low Perplexity &            0.692 &           0.854 &          0.823 &        0.039 &    0.032 \\
              &        & PromptSource &            0.768 &           0.854 &          0.821 &        0.038 &    0.036 \\
              &        & Null Instruction &            0.720 &           0.852 &          0.812 &        0.041 &    0.038 \\
              &        & RLPrompt &            0.712 &           0.850 &          0.813 &        0.042 &    0.034 \\
              & opt6b7 & APE &            0.684 &           0.878 &          0.855 &        0.032 &    0.026 \\
              &        & Ad hoc &            0.696 &           0.875 &          0.855 &        0.027 &    0.026 \\
              &        & Generic Instruction &            0.712 &           0.874 &          0.852 &        0.031 &    0.026 \\
              &        & Low Perplexity &            0.736 &           0.878 &          0.857 &        0.029 &    0.026 \\
              &        & PromptSource &            0.740 &           0.877 &          0.858 &        0.028 &    0.027 \\
              &        & Null Instruction &            0.680 &           0.869 &          0.852 &        0.031 &    0.025 \\
              &        & RLPrompt &            0.644 &           0.870 &          0.844 &        0.027 &    0.025 \\
NQ-Open & bloom1b1 & APE &            0.008 &           0.036 &          0.028 &        0.019 &    0.011 \\
              &        & Ad hoc &            0.012 &           0.038 &          0.031 &        0.021 &    0.008 \\
              &        & Generic Instruction &            0.012 &           0.037 &          0.029 &        0.020 &    0.008 \\
              &        & Low Perplexity &            0.012 &           0.037 &          0.028 &        0.020 &    0.008 \\
              &        & PromptSource &            0.008 &           0.038 &          0.029 &        0.020 &    0.008 \\
              &        & Null Instruction &            0.000 &           0.036 &          0.033 &        0.019 &    0.011 \\
              & bloom1b7 & APE &            0.028 &           0.074 &          0.070 &        0.018 &    0.014 \\
              &        & Ad hoc &            0.036 &           0.074 &          0.067 &        0.021 &    0.012 \\
              &        & Generic Instruction &            0.032 &           0.074 &          0.068 &        0.020 &    0.013 \\
              &        & Low Perplexity &            0.032 &           0.074 &          0.066 &        0.019 &    0.011 \\
              &        & PromptSource &            0.040 &           0.074 &          0.066 &        0.018 &    0.012 \\
              &        & Null Instruction &            0.020 &           0.075 &          0.069 &        0.018 &    0.010 \\
              & bloom3b & APE &            0.048 &           0.071 &          0.073 &        0.015 &    0.010 \\
              &        & Ad hoc &            0.044 &           0.072 &          0.070 &        0.015 &    0.009 \\
              &        & Generic Instruction &            0.044 &           0.069 &          0.074 &        0.013 &    0.007 \\
              &        & Low Perplexity &            0.060 &           0.071 &          0.067 &        0.015 &    0.010 \\
              &        & PromptSource &            0.052 &           0.070 &          0.071 &        0.014 &    0.008 \\
              &        & Null Instruction &            0.060 &           0.076 &          0.075 &        0.017 &    0.009 \\
              & bloom7b1 & APE &            0.056 &           0.116 &          0.101 &        0.015 &    0.009 \\
              &        & Ad hoc &            0.040 &           0.116 &          0.102 &        0.016 &    0.009 \\
              &        & Generic Instruction &            0.040 &           0.115 &          0.105 &        0.016 &    0.008 \\
              &        & Low Perplexity &            0.060 &           0.115 &          0.102 &        0.015 &    0.008 \\
              &        & PromptSource &            0.048 &           0.119 &          0.103 &        0.016 &    0.008 \\
              &        & Null Instruction &            0.040 &           0.112 &          0.099 &        0.015 &      0.000 \\
              & gptneo1b3 & APE &            0.040 &           0.093 &          0.075 &        0.024 &    0.008 \\
              &        & Ad hoc &            0.040 &           0.086 &          0.071 &        0.025 &    0.011 \\
              &        & Generic Instruction &            0.032 &           0.086 &          0.074 &        0.025 &    0.007 \\
              &        & Low Perplexity &            0.032 &           0.089 &          0.073 &        0.022 &    0.010 \\
              &        & PromptSource &            0.040 &           0.088 &          0.074 &        0.023 &    0.011 \\
              &        & Null Instruction &            0.040 &           0.088 &          0.075 &        0.027 &    0.009 \\
              & gptneo2b7 & APE &            0.008 &           0.082 &          0.046 &        0.019 &    0.010 \\
              &        & Ad hoc &            0.008 &           0.088 &          0.053 &        0.020 &    0.009 \\
              &        & Generic Instruction &            0.008 &           0.085 &          0.049 &        0.020 &    0.012 \\
              &        & Low Perplexity &            0.000 &           0.085 &          0.051 &        0.021 &    0.012 \\
              &        & PromptSource &            0.016 &           0.085 &          0.050 &        0.019 &    0.008 \\
              &        & Null Instruction &            0.000 &           0.087 &          0.049 &        0.021 &    0.006 \\
              & gptneox20b & APE &            0.064 &           0.143 &          0.112 &        0.027 &    0.014 \\
              &        & Ad hoc &            0.072 &           0.133 &          0.103 &        0.033 &    0.016 \\
              &        & Generic Instruction &            0.072 &           0.143 &          0.110 &        0.029 &    0.017 \\
              &        & Low Perplexity &            0.080 &           0.139 &          0.112 &        0.029 &    0.017 \\
              &        & PromptSource &            0.096 &           0.140 &          0.111 &        0.030 &    0.015 \\
              &        & Null Instruction &            0.100 &           0.137 &          0.105 &        0.021 &    0.017 \\
              & llama13b & APE &            0.332 &           0.365 &          0.379 &        0.019 &    0.013 \\
              &        & Ad hoc &            0.320 &           0.369 &          0.375 &        0.020 &    0.014 \\
              &        & Generic Instruction &            0.320 &           0.367 &          0.378 &        0.020 &    0.015 \\
              &        & Low Perplexity &            0.320 &           0.371 &          0.383 &        0.022 &    0.015 \\
              &        & PromptSource &            0.312 &           0.370 &          0.380 &        0.021 &    0.013 \\
              &        & Null Instruction &            0.220 &           0.368 &          0.381 &        0.020 &    0.019 \\
              & llama7b & APE &            0.144 &           0.260 &          0.231 &        0.022 &    0.019 \\
              &        & Ad hoc &            0.092 &           0.261 &          0.229 &        0.021 &    0.020 \\
              &        & Generic Instruction &            0.056 &           0.263 &          0.230 &        0.022 &    0.019 \\
              &        & Low Perplexity &            0.136 &           0.258 &          0.226 &        0.023 &    0.020 \\
              &        & PromptSource &            0.136 &           0.261 &          0.230 &        0.025 &    0.018 \\
              &        & Null Instruction &            0.120 &           0.255 &          0.225 &        0.021 &    0.020 \\
              & opt13b & APE &            0.072 &           0.187 &          0.160 &        0.031 &    0.014 \\
              &        & Ad hoc &            0.100 &           0.188 &          0.155 &        0.032 &    0.015 \\
              &        & Generic Instruction &            0.084 &           0.185 &          0.159 &        0.033 &    0.014 \\
              &        & Low Perplexity &            0.096 &           0.192 &          0.164 &        0.034 &    0.014 \\
              &        & PromptSource &            0.128 &           0.190 &          0.159 &        0.032 &    0.014 \\
              &        & Null Instruction &            0.020 &           0.187 &          0.168 &        0.033 &    0.015 \\
              & opt1b3 & APE &            0.036 &           0.081 &          0.053 &        0.027 &    0.016 \\
              &        & Ad hoc &            0.032 &           0.082 &          0.052 &        0.027 &    0.018 \\
              &        & Generic Instruction &            0.024 &           0.086 &          0.054 &        0.026 &    0.017 \\
              &        & Low Perplexity &            0.044 &           0.084 &          0.051 &        0.028 &    0.017 \\
              &        & PromptSource &            0.032 &           0.085 &          0.051 &        0.026 &    0.016 \\
              &        & Null Instruction &            0.040 &           0.089 &          0.053 &        0.032 &    0.017 \\
              & opt2b7 & APE &            0.052 &           0.130 &          0.104 &        0.022 &    0.008 \\
              &        & Ad hoc &            0.060 &           0.126 &          0.101 &        0.023 &    0.007 \\
              &        & Generic Instruction &            0.048 &           0.131 &          0.101 &        0.021 &    0.008 \\
              &        & Low Perplexity &            0.044 &           0.126 &          0.101 &        0.023 &    0.008 \\
              &        & PromptSource &            0.052 &           0.130 &          0.103 &        0.024 &    0.008 \\
              &        & Null Instruction &            0.020 &           0.123 &          0.104 &        0.017 &    0.010 \\
              & opt6b7 & APE &            0.108 &           0.185 &          0.141 &        0.030 &    0.013 \\
              &        & Ad hoc &            0.056 &           0.180 &          0.139 &        0.034 &    0.015 \\
              &        & Generic Instruction &            0.080 &           0.183 &          0.138 &        0.027 &    0.014 \\
              &        & Low Perplexity &            0.096 &           0.183 &          0.141 &        0.030 &    0.014 \\
              &        & PromptSource &            0.108 &           0.183 &          0.145 &        0.028 &    0.013 \\
              &        & Null Instruction &            0.100 &           0.183 &          0.135 &        0.037 &    0.012 \\
TriviaQA & bloom1b1 & APE &            0.020 &           0.114 &          0.119 &        0.031 &    0.015 \\
              &        & Ad hoc &            0.032 &           0.114 &          0.112 &        0.029 &    0.012 \\
              &        & Generic Instruction &            0.040 &           0.111 &          0.116 &        0.029 &    0.011 \\
              &        & Low Perplexity &            0.020 &           0.113 &          0.113 &        0.027 &    0.014 \\
              &        & PromptSource &            0.052 &           0.113 &          0.115 &        0.027 &    0.013 \\
              &        & Null Instruction &            0.100 &           0.116 &          0.116 &        0.028 &    0.013 \\
              & bloom1b7 & APE &            0.064 &           0.162 &          0.130 &        0.026 &    0.013 \\
              &        & Ad hoc &            0.076 &           0.166 &          0.133 &        0.025 &    0.011 \\
              &        & Generic Instruction &            0.072 &           0.166 &          0.131 &        0.024 &    0.013 \\
              &        & Low Perplexity &            0.068 &           0.164 &          0.130 &        0.027 &    0.013 \\
              &        & PromptSource &            0.108 &           0.165 &          0.131 &        0.027 &    0.012 \\
              &        & Null Instruction &            0.060 &           0.171 &          0.129 &        0.027 &    0.013 \\
              & bloom3b & APE &            0.136 &           0.209 &          0.201 &        0.023 &    0.020 \\
              &        & Ad hoc &            0.160 &           0.209 &          0.199 &        0.022 &    0.022 \\
              &        & Generic Instruction &            0.124 &           0.209 &          0.199 &        0.020 &    0.017 \\
              &        & Low Perplexity &            0.144 &           0.210 &          0.201 &        0.022 &    0.023 \\
              &        & PromptSource &            0.156 &           0.206 &          0.198 &        0.022 &    0.021 \\
              &        & Null Instruction &            0.100 &           0.213 &          0.207 &        0.022 &    0.023 \\
              & bloom7b1 & APE &            0.148 &           0.261 &          0.229 &        0.023 &    0.012 \\
              &        & Ad hoc &            0.148 &           0.263 &          0.233 &        0.024 &    0.010 \\
              &        & Generic Instruction &            0.144 &           0.267 &          0.230 &        0.023 &    0.008 \\
              &        & Low Perplexity &            0.144 &           0.265 &          0.232 &        0.021 &    0.012 \\
              &        & PromptSource &            0.156 &           0.263 &          0.229 &        0.019 &    0.012 \\
              &        & Null Instruction &            0.080 &           0.259 &          0.231 &        0.024 &    0.013 \\
              & gptneo1b3 & APE &            0.068 &           0.137 &          0.077 &        0.022 &    0.016 \\
              &        & Ad hoc &            0.076 &           0.137 &          0.076 &        0.020 &    0.016 \\
              &        & Generic Instruction &            0.072 &           0.138 &          0.079 &        0.021 &    0.016 \\
              &        & Low Perplexity &            0.072 &           0.137 &          0.077 &        0.020 &    0.015 \\
              &        & PromptSource &            0.100 &           0.136 &          0.076 &        0.020 &    0.015 \\
              &        & Null Instruction &            0.100 &           0.137 &          0.081 &        0.021 &    0.015 \\
              & gptneo2b7 & APE &            0.088 &           0.191 &          0.079 &        0.034 &    0.015 \\
              &        & Ad hoc &            0.088 &           0.192 &          0.085 &        0.041 &    0.018 \\
              &        & Generic Instruction &            0.100 &           0.189 &          0.085 &        0.035 &    0.017 \\
              &        & Low Perplexity &            0.096 &           0.188 &          0.086 &        0.039 &    0.015 \\
              &        & PromptSource &            0.116 &           0.190 &          0.081 &        0.037 &    0.017 \\
              &        & Null Instruction &            0.080 &           0.187 &          0.087 &        0.035 &    0.019 \\
              & gptneox20b & APE &            0.384 &           0.437 &          0.323 &        0.023 &    0.013 \\
              &        & Ad hoc &            0.376 &           0.437 &          0.320 &        0.027 &    0.013 \\
              &        & Generic Instruction &            0.384 &           0.442 &          0.326 &        0.021 &    0.008 \\
              &        & Low Perplexity &            0.393 &           0.437 &          0.321 &        0.023 &    0.012 \\
              &        & PromptSource &            0.396 &           0.442 &          0.322 &        0.021 &    0.015 \\
              &        & Null Instruction &            0.380 &           0.443 &          0.327 &        0.017 &    0.008 \\
              & llama13b & APE &            0.600 &           0.622 &          0.543 &        0.020 &    0.009 \\
              &        & Ad hoc &            0.568 &           0.626 &          0.547 &        0.021 &    0.007 \\
              &        & Generic Instruction &            0.592 &           0.624 &          0.548 &        0.022 &    0.005 \\
              &        & Low Perplexity &            0.508 &           0.624 &          0.550 &        0.022 &    0.008 \\
              &        & PromptSource &            0.584 &           0.625 &          0.546 &        0.020 &    0.007 \\
              &        & Null Instruction &            0.520 &           0.629 &          0.548 &        0.020 &      0.000 \\
              & llama7b & APE &            0.476 &           0.578 &          0.419 &        0.048 &    0.015 \\
              &        & Ad hoc &            0.452 &           0.589 &          0.422 &        0.045 &    0.018 \\
              &        & Generic Instruction &            0.384 &           0.585 &          0.419 &        0.047 &    0.015 \\
              &        & Low Perplexity &            0.464 &           0.592 &          0.421 &        0.045 &    0.018 \\
              &        & PromptSource &            0.464 &           0.584 &          0.424 &        0.046 &    0.016 \\
              &        & Null Instruction &            0.400 &           0.585 &          0.411 &        0.049 &    0.017 \\
              & opt13b & APE &            0.328 &           0.334 &          0.236 &        0.026 &    0.012 \\
              &        & Ad hoc &            0.308 &           0.338 &          0.238 &        0.023 &    0.012 \\
              &        & Generic Instruction &            0.304 &           0.339 &          0.228 &        0.022 &    0.011 \\
              &        & Low Perplexity &            0.304 &           0.338 &          0.235 &        0.024 &    0.011 \\
              &        & PromptSource &            0.332 &           0.337 &          0.235 &        0.025 &    0.012 \\
              &        & Null Instruction &            0.300 &           0.339 &          0.235 &        0.018 &    0.012 \\
              & opt1b3 & APE &            0.096 &           0.241 &          0.168 &        0.025 &    0.015 \\
              &        & Ad hoc &            0.092 &           0.237 &          0.162 &        0.030 &    0.014 \\
              &        & Generic Instruction &            0.108 &           0.239 &          0.164 &        0.028 &    0.015 \\
              &        & Low Perplexity &            0.096 &           0.239 &          0.163 &        0.025 &    0.016 \\
              &        & PromptSource &            0.132 &           0.234 &          0.160 &        0.028 &    0.015 \\
              &        & Null Instruction &            0.060 &           0.235 &          0.160 &        0.031 &    0.014 \\
              & opt2b7 & APE &            0.184 &           0.284 &          0.226 &        0.022 &    0.013 \\
              &        & Ad hoc &            0.176 &           0.282 &          0.218 &        0.018 &    0.013 \\
              &        & Generic Instruction &            0.176 &           0.281 &          0.222 &        0.021 &    0.018 \\
              &        & Low Perplexity &            0.152 &           0.281 &          0.219 &        0.019 &    0.015 \\
              &        & PromptSource &            0.204 &           0.282 &          0.224 &        0.021 &    0.018 \\
              &        & Null Instruction &            0.140 &           0.283 &          0.228 &        0.021 &    0.020 \\
              & opt6b7 & APE &            0.256 &           0.360 &          0.263 &        0.022 &    0.016 \\
              &        & Ad hoc &            0.236 &           0.361 &          0.258 &        0.020 &    0.018 \\
              &        & Generic Instruction &            0.260 &           0.363 &          0.255 &        0.025 &    0.019 \\
              &        & Low Perplexity &            0.280 &           0.361 &          0.260 &        0.024 &    0.019 \\
              &        & PromptSource &            0.292 &           0.362 &          0.256 &        0.022 &    0.019 \\
              &        & Null Instruction &            0.240 &           0.364 &          0.259 &        0.023 &    0.016 \\
Emotion & bloom1b1 & APE &            0.372 &           0.332 &          0.324 &        0.063 &    0.067 \\
              &        & Ad hoc &            0.368 &           0.319 &          0.317 &        0.063 &    0.053 \\
              &        & Generic Instruction &            0.340 &           0.338 &          0.330 &        0.065 &    0.083 \\
              &        & Low Perplexity &            0.352 &           0.303 &          0.297 &        0.059 &    0.038 \\
              &        & PromptSource &            0.328 &           0.313 &          0.309 &        0.059 &    0.049 \\
              &        & Null Instruction &            0.340 &           0.333 &          0.323 &        0.055 &    0.082 \\
              &        & RLPrompt &            0.352 &           0.334 &          0.327 &        0.065 &    0.090 \\
              & bloom1b7 & APE &            0.352 &           0.406 &          0.385 &        0.090 &    0.057 \\
              &        & Ad hoc &            0.300 &           0.363 &          0.347 &        0.082 &    0.051 \\
              &        & Generic Instruction &            0.368 &           0.401 &          0.373 &        0.086 &    0.062 \\
              &        & Low Perplexity &            0.276 &           0.356 &          0.335 &        0.083 &    0.050 \\
              &        & PromptSource &            0.312 &           0.374 &          0.353 &        0.075 &    0.056 \\
              &        & Null Instruction &            0.260 &           0.415 &          0.400 &        0.099 &    0.058 \\
              &        & RLPrompt &            0.352 &           0.410 &          0.398 &        0.085 &    0.057 \\
              & bloom3b & APE &            0.372 &           0.389 &          0.387 &        0.067 &    0.069 \\
              &        & Ad hoc &            0.344 &           0.326 &          0.332 &        0.059 &    0.040 \\
              &        & Generic Instruction &            0.420 &           0.424 &          0.419 &        0.079 &    0.095 \\
              &        & Low Perplexity &            0.308 &           0.297 &          0.308 &        0.048 &    0.027 \\
              &        & PromptSource &            0.392 &           0.340 &          0.344 &        0.063 &    0.039 \\
              &        & Null Instruction &            0.360 &           0.457 &          0.455 &        0.082 &    0.103 \\
              &        & RLPrompt &            0.376 &           0.415 &          0.414 &        0.080 &    0.099 \\
              & bloom7b1 & APE &            0.392 &           0.442 &          0.426 &        0.065 &    0.062 \\
              &        & Ad hoc &            0.384 &           0.389 &          0.370 &        0.052 &    0.040 \\
              &        & Generic Instruction &            0.420 &           0.465 &          0.439 &        0.085 &    0.064 \\
              &        & Low Perplexity &            0.320 &           0.376 &          0.355 &        0.066 &    0.043 \\
              &        & PromptSource &            0.356 &           0.404 &          0.381 &        0.065 &    0.043 \\
              &        & Null Instruction &            0.400 &           0.484 &          0.459 &        0.080 &    0.077 \\
              &        & RLPrompt &            0.420 &           0.487 &          0.454 &        0.079 &    0.069 \\
              & gptneo1b3 & APE &            0.324 &           0.365 &          0.355 &        0.068 &    0.041 \\
              &        & Ad hoc &            0.352 &           0.308 &          0.298 &        0.043 &    0.015 \\
              &        & Generic Instruction &            0.312 &           0.379 &          0.370 &        0.065 &    0.046 \\
              &        & Low Perplexity &            0.304 &           0.290 &          0.281 &        0.035 &    0.009 \\
              &        & PromptSource &            0.360 &           0.306 &          0.301 &        0.041 &    0.014 \\
              &        & Null Instruction &            0.280 &           0.387 &          0.377 &        0.070 &    0.050 \\
              &        & RLPrompt &            0.316 &           0.376 &          0.370 &        0.062 &    0.047 \\
              & gptneo2b7 & APE &            0.296 &           0.450 &          0.447 &        0.074 &    0.062 \\
              &        & Ad hoc &            0.404 &           0.432 &          0.424 &        0.086 &    0.059 \\
              &        & Generic Instruction &            0.272 &           0.463 &          0.454 &        0.091 &    0.060 \\
              &        & Low Perplexity &            0.332 &           0.423 &          0.423 &        0.084 &    0.055 \\
              &        & PromptSource &            0.372 &           0.419 &          0.415 &        0.087 &    0.051 \\
              &        & Null Instruction &            0.260 &           0.460 &          0.452 &        0.097 &    0.051 \\
              &        & RLPrompt &            0.292 &           0.458 &          0.450 &        0.086 &    0.067 \\
              & gptneox20b & APE &            0.384 &           0.553 &          0.512 &        0.072 &    0.047 \\
              &        & Ad hoc &            0.304 &           0.523 &          0.499 &        0.079 &    0.045 \\
              &        & Generic Instruction &            0.384 &           0.555 &          0.487 &        0.073 &    0.046 \\
              &        & Low Perplexity &            0.280 &           0.572 &          0.559 &        0.077 &    0.055 \\
              &        & PromptSource &            0.300 &           0.550 &          0.538 &        0.074 &    0.052 \\
              &        & Null Instruction &            0.420 &           0.559 &          0.507 &        0.054 &    0.040 \\
              &        & RLPrompt &            0.396 &           0.543 &          0.493 &        0.077 &    0.043 \\
              & llama13b & APE &            0.448 &           0.638 &          0.616 &        0.040 &    0.031 \\
              &        & Ad hoc &            0.320 &           0.604 &          0.576 &        0.059 &    0.034 \\
              &        & Generic Instruction &            0.456 &           0.635 &          0.622 &        0.045 &    0.035 \\
              &        & Low Perplexity &            0.336 &           0.602 &          0.579 &        0.052 &    0.033 \\
              &        & PromptSource &            0.444 &           0.610 &          0.591 &        0.052 &    0.035 \\
              &        & Null Instruction &            0.480 &           0.647 &          0.635 &        0.052 &      0.000 \\
              &        & RLPrompt &            0.452 &           0.649 &          0.633 &        0.050 &    0.035 \\
              & llama7b & APE &            0.384 &           0.596 &          0.594 &        0.053 &    0.039 \\
              &        & Ad hoc &            0.312 &           0.567 &          0.553 &        0.053 &    0.042 \\
              &        & Generic Instruction &            0.380 &           0.600 &          0.611 &        0.049 &    0.036 \\
              &        & Low Perplexity &            0.284 &           0.587 &          0.590 &        0.049 &    0.037 \\
              &        & PromptSource &            0.412 &           0.599 &          0.598 &        0.049 &    0.034 \\
              &        & Null Instruction &            0.420 &           0.608 &          0.613 &        0.038 &    0.035 \\
              &        & RLPrompt &            0.396 &           0.591 &          0.600 &        0.055 &    0.036 \\
              & opt13b & APE &            0.308 &           0.531 &          0.511 &        0.053 &    0.041 \\
              &        & Ad hoc &            0.424 &           0.525 &          0.495 &        0.057 &    0.053 \\
              &        & Generic Instruction &            0.308 &           0.534 &          0.522 &        0.041 &    0.039 \\
              &        & Low Perplexity &            0.488 &           0.531 &          0.495 &        0.068 &    0.071 \\
              &        & PromptSource &            0.432 &           0.542 &          0.514 &        0.067 &    0.060 \\
              &        & Null Instruction &            0.300 &           0.515 &          0.503 &        0.055 &    0.032 \\
              &        & RLPrompt &            0.320 &           0.536 &          0.522 &        0.050 &    0.035 \\
              & opt1b3 & APE &            0.344 &           0.385 &          0.382 &        0.074 &    0.057 \\
              &        & Ad hoc &            0.376 &           0.366 &          0.357 &        0.057 &    0.043 \\
              &        & Generic Instruction &            0.364 &           0.417 &          0.409 &        0.090 &    0.062 \\
              &        & Low Perplexity &            0.312 &           0.311 &          0.313 &        0.040 &    0.023 \\
              &        & PromptSource &            0.352 &           0.365 &          0.361 &        0.067 &    0.042 \\
              &        & Null Instruction &            0.300 &           0.411 &          0.412 &        0.071 &    0.056 \\
              &        & RLPrompt &            0.396 &           0.420 &          0.414 &        0.079 &    0.063 \\
              & opt2b7 & APE &            0.284 &           0.394 &          0.384 &        0.083 &    0.050 \\
              &        & Ad hoc &            0.308 &           0.354 &          0.345 &        0.074 &    0.049 \\
              &        & Generic Instruction &            0.332 &           0.433 &          0.411 &        0.078 &    0.053 \\
              &        & Low Perplexity &            0.284 &           0.391 &          0.385 &        0.100 &    0.068 \\
              &        & PromptSource &            0.332 &           0.359 &          0.356 &        0.083 &    0.048 \\
              &        & Null Instruction &            0.280 &           0.432 &          0.420 &        0.080 &    0.044 \\
              &        & RLPrompt &            0.280 &           0.432 &          0.411 &        0.080 &    0.051 \\
              & opt6b7 & APE &            0.352 &           0.441 &          0.426 &        0.064 &    0.037 \\
              &        & Ad hoc &            0.436 &           0.474 &          0.452 &        0.060 &    0.043 \\
              &        & Generic Instruction &            0.380 &           0.466 &          0.454 &        0.061 &    0.034 \\
              &        & Low Perplexity &            0.576 &           0.480 &          0.443 &        0.051 &    0.050 \\
              &        & PromptSource &            0.472 &           0.455 &          0.437 &        0.055 &    0.036 \\
              &        & Null Instruction &            0.300 &           0.460 &          0.440 &        0.074 &    0.029 \\
              &        & RLPrompt &            0.348 &           0.465 &          0.455 &        0.058 &    0.040 \\
\end{supertabular}


==> tables/methods_and_instructions.tex <==
\begin{table*}[t] 
\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{lccl}
\toprule 
\large \textbf{Method} & \large \textbf{Task-specific} & \large \textbf{Automatic induction} 
 & \large \textbf{Example instruction}\\ 

\midrule
\large{Null instruction} & \xmark & \xmark & (empty string)\\
\large{Generic instruction} & \xmark & \xmark & \texttt{Solve the following task:}\\
\midrule
\large{PromptSource} \cite{promptsource} & \cmark & \xmark & \texttt{What label best describes this news article?} \\
\large{Ad hoc} & \cmark & \xmark & \texttt{Which newspaper section is most likely to} \\ & & & \texttt{feature this news article?} \\
\midrule
\large{Low Perplexity} \cite{lowperplexityprompts} & \cmark & \cmark & \texttt{Which part of a newspaper do you think this} \\ & & & \texttt{article belongs to? World News, Sports, Business} \\
& & & \texttt{or Science and Technology?}\\
\large{APE} \cite{ape} & \cmark & \cmark & \texttt{classify each input into one of the following} \\ 
& & &\texttt{categories: World, U.S., Business, Sci/Tech,} \\ & & & \texttt{or Sports.}\\
\large{RLPrompt} \cite{rlprompt} & \cmark & \cmark & \texttt{Tools undergradCam firmwareCam} \\
\bottomrule
\end{tabular}}
\caption{Characteristics of instruction selection methods we consider}
\label{table:methods_and_instructions}
\end{table*}

==> tables/tasks_and_templates.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Task Type} & \textbf{Tasks}  & \textbf{Demonstration template}     \\ 
\midrule
\multirow{5}{*}{Classification (CLS)}      & AG News \cite{agnews} & \texttt{News: }(text)\texttt{\textbackslash nCategory: }(label)\\ 
& ANLI \cite{anli} & \texttt{Premise: }(premise)\texttt{\textbackslash nHypothetisis: }(hypothesis)\texttt{\textbackslash nRelation: }(label) \\
                                            & BoolQ \cite{boolq} & \texttt{Passage: }(passage)\texttt{\textbackslash nQuestion: }(question) \texttt{\textbackslash nAnswer: }(label) \\ 
                                            & IMDB \cite{imdb} & \texttt{Review: }(text)\texttt{\textbackslash nSentiment: }(label) \\ 
                                            & TweetEval Emotion \cite{emotion} & \texttt{Tweet: }(text)\texttt{\textbackslash nEmotion: }(label)\\
\midrule                                            
\multirow{2}{*}{Multiple-choice (MCQ)}                      & CosmosQA \cite{cosmosqa} & \texttt{Passage: }(context)\texttt{\textbackslash nQuestion: }(question)\texttt{\textbackslash nAnswer: }(answer) \\ 
& HellaSwag \cite{hellaswag}  & \texttt{Sentence: }(ctx)\texttt{\textbackslash nAnswer: }(answer) \\
\midrule
\multirow{2}{*}{Generative QA (GQA)}                         & NQ-Open \cite{nqopen} & \texttt{Question: }(question)\texttt{\textbackslash nAnswer: }(answer)\\ 
& TriviaQA \cite{triviaqa} & \texttt{Question: }(question)\texttt{\textbackslash nAnswer: }(answer)  \\ \bottomrule
\end{tabular}}
\caption{Tasks included in our evaluation suite, and the demonstrations templates we use for each task.}
\label{table:tasks_and_templates}
\end{table*}
